Computing Threshold Circuits with Void Reactions in Step Chemical Reaction Networks

We introduce a new model of \emph{step} Chemical Reaction Networks (step CRNs), motivated by the step-wise addition of materials in standard lab procedures. Step CRNs have ordered reactants that transform into products via reaction rules over a series of steps. We study an important subset of weak reaction rules, \emph{void} rules, in which chemical species may only be deleted but never changed. We demonstrate the capabilities of these simple limited systems to simulate threshold circuits and compute functions using various configurations of rule sizes and step constructions, and prove that without steps, void rules are incapable of these computations, which further motivates the step model. Additionally, we prove the coNP-completeness of verifying if a given step CRN computes a function, holding even for $O(1)$ step systems.

==> 2_0_formulas.tex <==
\section{Computation of Formulas with (2, 0) Rules}\label{2_0_formulas}

Having established compatibility results with stepped CRNs with (3, 0) rules, we now examine stepped CRNs with a ruleset consisting of (2, 0) rules instead. Decreasing the reactant count of the void rules has some notable changes to the system's computation.

Section \ref{2_0_gates} shows how the computation of logic gates is still possible in stepped CRNs with (2, 0) rules. We then demonstrate with Theorem \ref{(2,0)_formula} how the system can compute TC \textit{formulas} (but not circuits) with $O$($G$) species, $O$($D$) steps, and $O$($G$) volume.

\subsection{Computing Logic Gates}\label{2_0_gates}
%(2, 0) CRN's are not capable of hard coding a two-input gate. We can not consider both inputs and destroy an output based on them. This limits us to reactions that can only include one of the inputs. Our solution is achieved by manipulating the outputs. given an and gate, any 1 input deletes a 0 output, and any 0 input deletes a 1 output. The number of 0 outputs is equal to the number of inputs because all inputs must be 1 for an and gate to not return 0.

The inputs of a binary gate in a step CRN system are constructed the same as in Section \ref{3_0_gates}. Let $f_i^{in}$ be the set of all the indexes of the inputs fanning into a gate at index $i$. Let $f_i^{out}$ be the set of all the indexes of the inputs fanning out of a gate at index $i$.

The outputs of gates in a step CRN system with (2, 0) rules are represented by either the species $y_n^b$ or $y_{i \rightarrow j}^F$.

\subsubsection{Basic Gates}\label{2_0_basic_gates}

Computing gates with (2, 0) rules requires a unique species to represent the inputs and outputs of each gate in a circuit. The species used to compute a particular gate should never be used to compute a different gate. Figure \ref{fig:(3,0)_figure} \textit{(b)} shows a pattern the gates can be indexed in. To compute an AND gate, we add a single copy of the species representing a true output ($y_{j}^T$) and a species representing the false output for each input fanning in ($y_{i \rightarrow j}^F$, where $i$ is the index of the input). To compute an OR gate, we would add a species representing the true output for each input fanning in ($y_{i \rightarrow j}^T$) species and a single $y_{j}^F$ species. To compute NOT gates, we would just add one copy of each output species. For all AND/OR/NOT gates, a rule should be made for every input fanning into a particular gate to delete the gate's output species with the opposite truth value to the input. If the output species has a unique $i \rightarrow j$ indexing, then only the input with the $i$th index can delete that output species.

\begin{table}[H]
\begin{center}
\begin{tabular}{| c | c | c |}\hline
\textbf{AND Gate} & \textbf{OR Gate} & \textbf{NOT Gate} \\ \hline

$x_i^T + y_{i \rightarrow j}^F \rightarrow \emptyset$ & $x_i^T + y_j^F \rightarrow \emptyset$ & $x_i^T + y_j^T \rightarrow \emptyset$ \\ \hline
 
$x_i^F + y_j^T \rightarrow \emptyset$ & $x_i^F + y_{i \rightarrow j}^T \rightarrow \emptyset$ & $x_i^F + y_j^F \rightarrow \emptyset$ \\ \hline


\end{tabular}

\caption{\textit{(2, 0) rules for AND, OR, and NOT gates.}}\label{tab:(2,0)_AND_OR_NOT}
\end{center}
\end{table}

\subsubsection{Majority Gate}\label{2_0_majority_gates}

Let's consider the majority function when it has two unique input species, $T$ and $F$, where the counts of each species represent the amounts of true and false inputs, respectively. If $(|T| + |F|) \% 2 = 0$, then we should add an extra $F$ species before computing.

To compute the majority function with (2, 0) rules, we add a rule where the T and F species delete each other: $T + F \rightarrow \emptyset$. With this rule, all of the minority species will be deleted and some amount of the majority species will remain.

To implement the majority gate in a circuit, given the inputs $x_i^b$ and output $y_i^b$, we must first convert the different input species into a new input species that share the same index before computing the majority function. If the amount of inputs fanning into a majority gate is even, then an extra false input should be fanned into that gate.

%To implement the majority gate in a circuit, we need to separate the input and output species. Instead of just the input species, $T$ and $F$, we also take the intermediate species $T_{i}$ and $F_{i}$. We also change our rules from $T + F \rightarrow \emptyset$ to $T_{i} + F \rightarrow \emptyset$ and $T + F_{i} \rightarrow \emptyset$.

%Before computing, if $(|T| + |F|) \% 2 = 0$, then we should add an extra $F_{i}$. To trigger the gate reaction we add in copies of each output species equal to half the input species, rounding down. After the rules are applied to this configuration, there will be either be only $F$ and $F_{i}$ or $T$ and $T_{i}$ To simplify the many $T_{i}$'s or $F_{i}$'s, we take a step.

%In the second step, we add one $T_{o}$ and one $F_{o}$ and execute the rules $T_{i} + F_{o} \rightarrow \emptyset$ and $F_{i} + T_{o} \rightarrow \emptyset$. This leaves us with either $T_{o}$ or $F_{0}$ representing our output.

To implement a majority gate in a circuit with (2, 0) rules, we must first convert all input species ($x_n^b$) fanning into the gate at index $i$ into a new species that share the same index, which we will call $a_i^b$. This will make it easier to compute the majority gate.

\begin{table}[H]
\begin{center}
\begin{tabular}{| c | c  c | c | c |}\hline

\multicolumn{3}{|c|}{\textbf{Steps}} & \textbf{Relevant Rules} & \textbf{Description} \\ \hline

\textbf{1} & \textit{Add} & \makecell{$|f_i^{in}| \cdot a_i^T$ \\ $|f_i^{in}| \cdot a_i^F$} 

& \makecell{\vspace{-10pt} \\ $\forall j \in f_i^{in}:$ \\ $x_j^T + a_i^F \rightarrow \emptyset$ \\ $x_j^F + a_i^T \rightarrow \emptyset$ \\ \vspace{-9pt}}

& \makecell{$\forall j \in f_i^{in}$, convert $x_{j}^b$ input \\ species into $a_i^b$ species.} \\ \hline

%%%
\textbf{2} & \textit{Add} & \makecell{$\lfloor |f_i^{in}|/2 \rfloor \cdot b_i^T$ \\ $\lfloor |f_i^{in}|/2 \rfloor \cdot b_i^F$} 

& \makecell{$a_i^T + b_i^F \rightarrow \emptyset$ \\ $a_i^F + b_i^T \rightarrow \emptyset$}

& \makecell{Adding $\lfloor |f_i^{in}|/2 \rfloor$ amounts of $b_i^T$ and \\ $b_i^F$ species will delete all of the \\ minority species, leaving some amount \\ of the majority species remaining.} \\ \hline

%%%
\textbf{3} & \textit{Add} & \makecell{\vspace{-8pt} \\ $y_i^T$ \\ $y_i^F$ \\ \vspace{-10pt}} 

& \makecell{$a_i^T + y_i^F \rightarrow \emptyset$ \\ $a_i^F + y_i^T \rightarrow \emptyset$}

& \makecell{Convert $a_i^b$ into the proper output \\ species ($y_i^b$).} \\ \hline

\end{tabular}

\caption{\textit{(2, 0) rules for majority gates.}}\label{tab:(2,0)_MAJ}
\end{center}
\end{table}



\subsection{Examples}\label{3_0_examples}

\begin{figure}[!htbp]
    \centering
    {\includegraphics[width=5cm]{images/2depthformula.pdf}
    
    \caption{Example Formula.}\label{fig:(2,0)_example}
    }
\end{figure}

\input{2_0_example}



\subsection{Computing Formulas (Multiple-Input Model)}\label{2_0_computation}

\begin{theorem}\label{(2,0)_formula}
Boolean formulas (TC) can be computed with multiple input relaxed by a step CRN with only $(2,0)$ rules, O(G) species, O(D) steps, and O(G) volume.
    \end{theorem}
\begin{proof}
%\textit 
%Formulas are circuits in combination with only 2 inputs and 1 output. 2,0 does this in O(D), specifically steps=D+1. Each gate has unique input and output species. each step represents 1 level being solved. The gates reactions are triggered by the output species added at each step. The first level runs with the gate rules discussed in the gate section with one edit. In the case of an AND gate, there is not 2 z0's. there is 1 z0, and 1 z0*. z0 reacts with x1 inputs, and z0* interacts with y1 inputs. This removes the possibility of a gate producing 2z0 and the next gate running the reaction z0+output1 twice. Then we add the output species for the second layer and that layer's rules run, then the next step triggers, repeat. At the final layer, after the gate is solved, we need to narrow our solution to one answer. This is done by adding running an inverted not gate, Z0+true, Z0'+true and Z1+false,Z1'+false. This leaves only true or false, a single species output.

Section \ref{2_0_gates} explains how to compute TC gates. In order to run the formula, we need to convert the outputs into the inputs for the next gate. This can be done in a step by adding $x_i^T$ and $x_i^F$ for each gate at a given depth level and applying the reactions below.

\begin{table}[H]
\begin{center}
\begin{tabular}{| c | c  c | c | c |}\hline

\multicolumn{3}{|c|}{\textbf{Steps}} & \textbf{Relevant Rules} & \textbf{Description} \\ \hline

\textbf{1} & \textit{Add} & \makecell{$x_i^T$ \\ $x_i^F$ \\} 

& \makecell{\vspace{-8pt} \\ $y_i^T + x_i^F \rightarrow \emptyset$ \\ $y_i^F + x_i^T \rightarrow \emptyset$ \\ $y_{j \rightarrow i}^T + x_i^F \rightarrow \emptyset$ \\ $y_{j \rightarrow i}^F + x_i^T \rightarrow \emptyset$ \\ \vspace{-8pt}}

& \makecell{Add species representing true and false \\ inputs and delete the species that are the \\ complement of the output. Now, only \\ the correct input species remains.} \\ \hline

\end{tabular}

\caption{\textit{(2, 0) rules for converting outputs to inputs per formula level.}}\label{tab:(2,0)_convert}
\end{center}
\end{table}

\textbf{Big-Oh Complexity Analysis:}
Having unique species to represent each gate in a Boolean formula results in O($G$) species.

All gates at a given depth level can be computed at the same time with a constant amount of steps, so a simulation of a Boolean formula would require O($D$) steps.

It is possible that not all species that are no longer needed will get deleted after computing a gate. For example, an AND gate with 3 false inputs would result in 3 $y_i^F$ and 2 false input species in the system. While this will not cause errors, it will increase the volume. Therefore, it is possible for only a fraction of the O($G$) species added throughout the simulation to be deleted, resulting in O($G$) volume.
\end{proof}

%REDUNDANT COROLLARY
%\begin{corollary}
%Fan-ins in Boolean formulas can be naturally simulated with only (2, 0) rules and no additional steps or species \textbf{(DOUBLE CHECK METRICS)}.
%\end{corollary}
%\begin{proof}
%\textit
%2,0 handles fan in by increasing the initial count of the outputs. for a five input and gate, there would be 5 z0's and 1 z1, with the rules (x,a means input a) x,1+z0->0 and x,0+z1->0 effectively, these inputs and rules ask the questions, are all inputs 1, and is at least one input 1. A 	single 0 input deletes z1 and leaves a z0 remaining. z0 is only entirely deleted if every input is 1.
%\end{proof}

==> abstract.tex <==
\begin{abstract}
We introduce the new model of \emph{step} Chemical Reaction Networks (step CRNs), motivated by the stepwise addition of materials in standard lab procedures, where ordered reactants transform into products via reaction rules. We study a subset of weak reaction rules, \emph{void} rules, in which chemical species may only be deleted but never changed or created. We show the capabilities of these systems to simulate circuits and compute functions using various configurations of rule sizes and step constructions.


% Chemical Reaction Networks (CRNs) are a fundamental model of computation in which a system of species changes over time through the application of replacement rules.  We present a straightforward augmentation of the model, motivated by standard lab practices, where a collection of new species may be added to the system once all reactions have finished. This process may continue over a sequence of discrete steps. We study the computational power of these \emph{step} CRNs under an extremely weak subset of CRNs in which reaction rules only delete species, i.e., never create any species.  These rules are termed \emph{void} rules and plausibly confer a substantially simpler and scalable molecular implementation.  Despite restrictions imposed by only using void rules, we show that such systems are capable of simulating general formulas and circuits within the step model.

% In particular, we show that void rules with three reactants and zero products ($(3,0)$ rules) can simulate Threshold Circuits (TC) of depth $D$ in $O(D\log D)$ steps, while void rules with only two reactants can also simulate TC in $O(D)$ steps if they can make use of catalysts.  We pair these positive results with a lower bound showing that, under our specified model of computation, computing general circuits requires more than a constant number of steps when not using catalysts.  We additionally consider the computational problem of verifying if a given step CRN computes a given function and show this problem is coNP-complete even for $O(1)$ step systems.



\end{abstract}

==> checklist.tex <==
Here is a list of feedback from reviewers.

When making changes on this paper, please:
1. Check off the item you fix
2. Briefly describe what you did to fix it underneath the item
3. Include your initials so we know who to bother if its not fixed right >:)

CHECKLIST
--------------------------------------------------------------------------------


FINISHED ITEMS
------------------------------------------------------------------------------------

(X) Change previous work references or wording: "while deterministic Chemical Reaction Networks can compute precisely the set of semilinear functions [4, 14]."
The references here are about population protocols and stochastic CRNs that have no error in output. The deterministic mass action model is Turing complete (it has been shown to be polynomially equivalent [see the papers below]). If you mean deterministic in the no-error stochastic sense, it would be good to clarify that. 
-Strong Turing Completeness of Continuous Chemical Reaction Networks and Compilation of Mixed Analog-Digital Programs
-Polynomial time corresponds to solutions of polynomial ordinary differential equations of polynomial length


(-) Reword preliminaries: The use of volume in Definition 3 as an alternative keyword for size may conflict for some readers with the physical volume of the solution a CRN is typically implemented it. it might be best to avoid overloading this word. As an alternative, perhaps use 'count'.
    -For now we just leaving it as is.

(-) Reorganize definitions: there are a lot of definitions that exist outside of a Definition # environment and there are often many definitions inside of each Definition # environment.
    -dont care


(X) Clarify preliminaries: "A strict step CRN computer" Why is computer appended to this here but not earlier? (You may also want to hyphenate CRN-computer to be consistent or remove the hypens that occur later) It seems like you want to say that a strict step CRN computer computes a function f if adding X(b) to $s_0$ causes it output Y(f(b)). Also, is there any intuition for what makes it strict? Might it not be better to call this an I/O step CRN or something of the like since you're defining how to give it input and read its output?
    Changed occurrences of step-CRN to step CRN. And CRN-computer to CRN computer.
    Added after explanation of input being 1 species for each input bit: "We consider this representation of the input to be strict, as opposed to allowing multiple copies of each input bit species." -RA

(x) Clarify preliminaries: "The corresponding step CRN $(Λ, Γ, (s_0 + X(b), . . . , s_{k−1}))$ is obtained by adding X(b) to $s_0$ in the first step."
What corresponding step CRN? A strict step CRN computer is just a step CRN with some species singled out. It seems like the authors are trying to say that the strict step CRN computer that this came from computes its function via this step CRN by adding the input to $s_0$. It might be good to state something to that effect or just let the definition of computes follow naturally later rather than pull this out of the aether without explaination.


(x) Clarify prelminaries: "A step CRN-computer strictly computes function f if" Why strictly computes? Is there a weaker notion of computation you use later? If so, why not go with computes and some analogous keyword (e.g. lower semicomputes) instead? Also, shouldn't this be a STRICT step CRN-computer?
-Added some explanation here - RTS
    Added after explanation of input being 1 species for each input bit: "We consider this representation of the input to be strict, as opposed to allowing multiple copies of each input bit species." -RA


(x) Reword Lemma 9: if the configuration distance is 1, then there is only one species where the occupation number is different in the two configurations and this proof becomes a bit simpler (there’s just T, not T and F). I think what you want is to say is the configuration distance is 2, or perhaps more specifically that the two configurations are encodings of bit strings with a Hamming distance of 1.
-They were correct, "1->2" 

(x) Introduction grammar: "and a set of a replacement rules" -> drop the a before 'a replacement rules'
    Removed a -RA

(x) Introduction grammar: the first discussions in 1988 [8], and an -> drop the comma
    Removed , -RA

(x) Introduction grammar: the sub module, however, if any product(s) -> change to '; however,' or '. However,'
    Used ". However," -RA

(x) Introduction grammar: if any product(s) remain they can -> you probably want a comma after remain
    Added , -RA

(x) Preliminaries grammar: a step CRN of k steps is a ordered -> AN ordered
    Changed a to an -RA

(x) Preliminaries grammar: which a are bounded by -> extra a
    Removed a -RA

(x) Preliminaries grammar: variable value, and subsequently assigning each -> no comma
    Removed , -RA

(x) Preliminaries grammar: be consistent with either multi-set or multiset
    Changed instances of multi-set to multiset -RA

(x) Preliminaries grammar: $s_0$, and $TERM_1$ the -> either lose the comma or preferably change to '$s_0$, and let $TERM_1$ be the'
    Used the second option -RA

(x) Preliminaries grammar: a void rule one whose product -> perhaps 'is one' or 'is a rule whose'?
    Used 'is a rule whose' -RA

(x) 3,0 section grammar: The general process to compute an AND -> you probably want AND gate to match the parenthetical OR gate
    added 'gate' after AND -RA

(x) Add definition: W was only ever defined in Table 1's caption. It might be good to define that elsewhere formally.
    Added definition of W to {sec:3_0_circuits} where it is first used in a big O result -RA

(x) Clarify indexing: "where n is the output bit index (input index of the level)"
input index of the next level? If not, I'm unsure what this means.
    Just added the word "next" -AS

(x) Change preliminaries order: When you define $REACH_{I,\Lambda,\Gamma}$, the I is undefined until the end of the paragraph. It would be best to have it defined up front.
    Moved the sentence defining I from the end of the paragraph to the beginning -RA

(x) Reword Lower Bound: "Similarly, define the species F." Not sure if this needs to be changed, but reading this tripped me up for a while.
    Lengthened this sentence to repeat much of the previous one, but in reverse: "Similarly, define the species $F$ to be the species in $c_F$ and not in $c_T$." -RA 

(x) Change introduction wording: The authors say a step CRN gives additional power to the standard CRN model, which is already Turing complete. perhaps it would be better to only have the part about it providing many useful techniques.
    Changed "give additional power to" to "extend" -RA

(x) Clarify preliminaries: "X(b) is defined as the configuration over Λ obtained by including 1 copy of $x^0_i$ if $b_i = 0$ and 1 copy of $x^1_i$ if $b_i$ = 1 for each bit $b_i$." Presumably, you also include 0 copies of the opposite species.
    Added the word "only", not sure how else to clarify this: "including 1 copy of x0i ONLY if bi = 0" and the same for x1i. -RA

(x) Reword preliminaries: "In this paper we only consider void rule systems which a are bounded by their nature."
Maybe just say 'bounded void rule systems'.
    Changed to bounded void rule systems -RA

(x) Preliminaries grammar: the union of all reachable configurations for each possible starting configuration -> from each possible?
    Changed "for" to "from" -RA

(x) Reorder Lower Bound: "In other words, the k-CNOT is a k-Lipschitz function."
Presumably, by k-Lipschitz function, the authors mean that the configuration distance (defined after) of the inputs and outputs satisfies $||f(X_1,Y_1) - f(X_2,Y_2)|| <= k||(X_1,Y_1) - (X_2,Y_2)||$. And this is true for f = k-CNOT since the maximum change f can produce is flipping every bit, which takes a configuration distance of 1 to a configuration distance of k. Regardless, defining the metric after implicitly using it is not great, especially since the k-Lipschitz keyword never gets used again.
    Commented out the mentioned sentence, as i am unsure where else we can easily make use of this keyword -RA

(x) Add to preliminaries: underscore that the $s_i$ values are all fixed for a fixed function f, so you can't cheat by doing outside computation to find $s_i$ values that produce f after you have your hands on the input.
    Added the following sentence to \subsection{Computing Functions in Step CRNs}: "For a fixed function $f$, the values denoted at each step $s_i$ are fixed to disallow outside computation." I am unsure if it should also be clarified when these values get fixed (at the beginning) or if this is clear enough -RA

(x) Reword preliminaries: "The fan-in 0 gates (source gates) are labeled from $x_1, x_2, . . . , x_n$, or from the constants 0 or 1."
It seems like the authors are trying to say that 'the fan-in 0 gates (source gates) are either the constants 0 and 1 or the variable vertices labelled $x_1, ..., x_n'$ or something to that effect. It reads a little awkwardly as is.
    Changed phrasing to "or labeled by constants starting at $0$ or $1$" as we are saying that we are starting from these constant numbers and counting upward to n or n-1, not that they are exclusively 0 or 1. -RA

(x) Clarify preliminaries: "Fan-out 0 gates may or may not be labeled as output gates."
While there is nothing prohibiting this, why would a gate that nothing depends on not either be an output gate or extirpated from the circuit?
    Commented out this sentence, but as the reviewer says theres nothing wrong with it and it could be added back in if needbe -RA

(x) Suggested add to introduction: A compelling use case for this model would be in medicine. For instance, a patient could take a pill day one, allow the reaction to proceed to completion, then take another pill on day two, and so on.
    Added to intro: "Another potential application for this model is in medicine, where a patient takes medication and then waits for reactions to complete before taking another medication". I would like to make this sentence less generic but the feedback is also generic -RA

    Alternative change: Changed the phrasing "...reflect laboratory practices..." to "...reflect laboratory and medical practices..." - A.M.

(x) Clarify lower bound: "The proof for this"
The proof for what? The demonstrative pronoun this is undefined. The authors are making an inductive argument about getting two end configurations with distance $2r^{s}$, but that was not indicated anywhere in the proof.
    Reordered sentence to remove the pronoun: "The proof for this follows the base case where each... so the species" to "In the base case, each... so it follows that the species" but left original sentence commented out -RA

(X) Change preliminaries term: The paper's ordered alphabet Lambda = ... should probably have braces around it unless you're explicitly treating it as a sequence since alphabets are usually sets.
    Added curly braces around the alphabet. - A.M.

(X) Add missing function: "and a Boolean function (footnote)1 where"
The paper is missing a function name to go with the footnote 1. Presumably it's supposed to be f.
    Added the term $f(\cdot)$ before the footnote. - A.M.

(X) Change preliminaries definition: The definition of rule/reaction gives two equivalent definitions back to back without explanation. It would probably best to either pick one (the vector representation is more common) or to start with one and say something to the effect of 'it can be equivalently represented as...'
    Deleted "A \emph{rule} or \emph{reaction} has two multisets, the first containing one or more \emph{reactant} (species) used for creating resulting \emph{product} (species) contained in the second multiset." This sentence came directly before the "vector" definition. -AS

(X) Change preliminaries syntax: Rather than use the squiggly arrow for the transitive closure of $\rightarrow^1_{Gamma}$, you might want to use $\rightarrow^*_{Gamma}$ or $\rightarrow^+_{Gamma}$ instead (depending if you want to include the no rule application).
    -Changed squiggly arrow to $\rightarrow^*_\Gamma$.
    Context: "We further use the notation $C\rightsquigarrow_\Gamma C'$ to signify the transitive closure..." -AS


(X) Reword preliminaries: Try to be consistent through the paper with the use of multiset versus set. For instance, in Definition 2, you say that the 'product set is a strict subset of the reactants', but both the reactions and products are multisets, so you would want a strict submultiset.
    Replaced "set" and "subset" with "multiset" and "submultiset", respectively. I think this was the only time products/reactants are referred to as "sets", so this definition is probably consistent at the moment. -AS


(X) Clarify preliminaries: formally define what a step is in a step CRN. From the abstract/introduction, it seems to be that a step is running a CRN to completion (i.e. to a terminal configuration), but this is not formally defined anywhere before you start using it. Figure 1 does not help determine if a step is, for example, a single reaction or running the system to completion. If it is running the system to completion, then how do you know with certainty that it's done? Certainly, you can get an arbitrarily high probability of certainity, but getting probability 1 is a different matter. It's known that a stochastic CRN can compute arbitrary circuits with an arbitrarily small chance of error, so the authors would want to either distinguish their paper from that or clarify that this is a refinement of that construction/alternative approach.
    In Introduction [1], modified "we augment the model with a sequence of discrete steps where an additional specified amount is combined with the existing CRN." and, in Setp CRNs [2.3], modified "A step CRN is an augmentation of a basic CRN in which additional copies of some system species are added after each of a sequence of steps." to specify when steps occur. -AS

(X) Clarify preliminaries: "by using initial configuration $s_{i−1}$"
Did you mean 'by using initial configuration $c_{i - 1}$ at step $s_{i - 1}'$? I suppose the s variables could be thought of as...augmenting initial conditions, because the c's are the terminal/next initial system state that you add s to.
    Changed the phrasing "...by using initial configuration $s_{i−1}$..." to "...by using initial configuration $c_{i - 1}$ at step $s_{i - 1}$..." - A.M.

==> reachability.tex <==
\section{Reachability}


\subsection{Size 2 Void Rules}

%%%%%%%%%%%%%
%2,0
%%%%%%%%%%%%%
\begin{theorem}
     Reachability for general CRNs with unary encoded species with only rules of size (2, 0) is in class P \cite{Alaniz:2022:ARXIV}.
\end{theorem}


\begin{theorem}\label{thm:20npc}
     Reachability for 2-step CRNs with only rules of size (2, 0) is NP-complete, even for unary encoded species counts.
\end{theorem}
\begin{proof}
Here, we reduce from the Minimum Maximal Matching problem, which is NP-complete even in a bipartite graph with max degree 3 \cite{Yannakakis:1980:SJAM}.
Given a positive integer $k$ and a bipartite graph $G=(L,R,E)$ where the two vertex sets $|L|=|R|$ and every edge is $\{l_i,r_j\} \in E$ s.t. $l_i \in L$ and $r_j \in R$. The minimum maximal matching problem asks whether there is a maximal matching of size $k$. For convenience, let $n=|L|$.
\begin{itemize}
    \item In the first step of the CRN, we create a species with one copy for every $l_i \in L$ and $r_j \in R$. For every edge $\{l_i,r_j\} \in E$, we create the rule $l_i + r_j \rightarrow \emptyset$.
    \item In step two, we add $2(n-k)$ copies of $D$, and the system has the rules $D + l_i \rightarrow \emptyset$ $\forall l_i \in L$, and $D + r_j \rightarrow \emptyset$ $\forall r_j \in R$.
\end{itemize}
In step 1, a maximal matching must be chosen by the rules since any reaction is essentially choosing an edge. If no more reactions are possible, then there are no more edges available with both vertex species in the system.

If there is a maximal matching of exactly size $k$, then there will be $2(n-k)$ vertices that are not part of the matching. Thus, the species representing those will still be in the system. The $D$ species will react with them and the final configuration will be $\emptyset$.

If the maximal matching is greater than $k$, there will be $D$ species left in the system. If the maximal matching is smaller than $k$, there will be vertex species remaining.
\end{proof}


%%%%%%%%%%%%%
%2,1
%%%%%%%%%%%%%

\begin{theorem}\label{thm:(2,1) rules}
    Reachability for general CRNs with size (2, 1) void rules is in NL
\end{theorem}
\begin{proof}
    Consider the implication graph $G$ where each node is a species $s_i$ and each reaction $s_i + s_j \rightarrow s_j$ implies a directed edge from $s_i$ to $s_j$. We will call any species with a target count of $\geq 1$ a root species. A species $s_i$ can be decreased from its initial count to its target count if and only if there exists a path in the implication graph from $s_i$ to a root species. This implies there exists a spanning forest each rooted at root nodes which can be used to reach the target configuration. Decreases the leaves of the spanning forest to their target counts then work up the trees. It is important to note this does not count self loops\footnote{Unless the self loop was added by a reaction such as $s_i + s_i \rightarrow s_i$} on root nodes that must be decreased. 

    This means an algorithm needs to make multiple calls to directed connectivity, which is solvable in NL. The algorithm checks the following for each species $s_j$ which decreases its count, check if there exists a path to any root node. If there does not exist a path then reject. If all species have a path then accept. This only requires $2$ points to the input so it is solvable in NL.  
\end{proof}


\begin{theorem} \label{thm:21npc}
     Reachability for 2-step CRNs with only rules of size (2, 1) is NP-complete, even for unary encoded species counts.
\end{theorem}
\begin{proof}
%\textit{I don't who's going to write this.}
We reduce from 3SAT. In the first step we introduce for each variable $x_i$ a pair of literal species $\{T_i, F_i\}$ each with initial count $1$ in the starting configuration. We also have a pair of assignment reactions for each $x_i$, one for true $T_i + F_i \rightarrow T_i$ and one for false $T_i + F_i \rightarrow F_i$. At the end of the first stage all variables must be assigned, deleting the non-assigned literal species. In the second step we will add a single copy of a clause species $C_j$ for each clause $c_j = (x_a, x_b, x_c)$. Each clause species will have $3$ verification reactions. Each of the form $C_j + T_a \rightarrow T_a$. If a literal is negated the reaction will be $C_j + F_b \rightarrow F_b$. The final species that is added in the second step is a single copy the clean up species $clean$. For each variable $x_i$ we have clean up reactions $clean + T_i \rightarrow clean$ and $clean + F_i \rightarrow clean$. Our target configuration is $\{ clean \}$.

If the 3SAT instance $\Phi$ is satisfiable then there exists an assignment $X$ which satisfies all the clauses. Using $X$ we may perform assignment reactions to reach a configuration at the end of the first stage which represents $X$. In the second stage since $X$ satisfies all the clauses, each clause species can be deleted with a verification reaction. Finally the clean up species can always delete all the literal species. Thus a solution to the 3SAT instance implies a solution to reconfiguration. 

If the target configuraiton is reachable then that means all clauses species were removed after being added to an intermediate configuration $Y$. Clause species can only be deleted by a verification reaction using one of its literal species as a catalyst. If all clause species have been deleted that means $Y$ contains at least one literal species that matches it. Since in the first stage we must make assignment to all the variables $Y$ implies a solution to $\Phi$. 
\end{proof}




\begin{corollary}\label{cor:2021npc}
    Reachability for 2-step CRNs with only void rules of size (2, 0) and (2, 1) is NP-complete, even for unary encoded species counts.
\end{corollary}
\begin{proof}
    Follows from Theorems \ref{thm:20npc} and \ref{thm:21npc}.
\end{proof}


\subsection{Size 3 Void Rules}
%%%%%%%%%%%%%
%3,1
%%%%%%%%%%%%%


\subsubsection{$(3,1)$ Void Rules}

\begin{figure}[t]
  \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=.9\textwidth]{images/hampath.png}
        \caption{}\label{fig:hamgraph}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \caption{}\label{fig:app}
    \end{subfigure}
    \caption{(a) Directed graph. (b)}\label{fig:31hamexample}
\end{figure}

Here, we show that with only $(3,1)$ void rules (one species in the reaction is a catalyst) in a regular CRN that reachability is NP-complete. We reduce from the Hamiltonian path problem in directed graphs. For simplicity, we reduce from the variation where each vertex has max in-degree and out-degree of two, which is still NP-complete \cite{Plesnik:1979:IPL}. We outline the species and then the reactions. We show correctness in the proof.

\paragraph{Species.} We are going to create a species for every path through a vertex (unless it starts at $t$ or goes back to $s$). Thus, looking at Figure \ref{fig:hamgraph}, for vertex $b$, we create two species $S_{a,b,c}$ and $S_{a,b,t}$. The notation being the vertex it came from, the vertex, and the vertex it goes to.  With max in/out degree of two, for each vertex, there are at most 4 paths through the vertex. In general, for each vertex $j$, we create the species $S_{i,j,k}$ where $(i,j),(j,k)\in E$ and $k \neq s$, $i\neq t$. For $s,t$, we just have $S_s$ and $S_t$.
We also create $P_i$ species for each $i\in V$ where $i\neq s$. Thus, we have $n-1$ of these species.



\paragraph{Reactions.} There are two main types of reactions: those that pick which path through a vertex and those that walk the Hamiltonian path.
\begin{itemize}
    \item Since there are at most 4 species per vertex, we will create rules that create a tournament to choose one of the species for each vertex. Assuming 3 species for ease of explanation, we create the rules $S_1 + S_2 + S_3 \rightarrow S_1$, $S_1 + S_2 + S_3 \rightarrow S_2$, and $S_1 + S_2 + S_3 \rightarrow S_3$. With only two species, we can create a dummy species that is not used as a catalyst. With 4 species, we augment the case of 3 species with another reaction that must occur with a dummy species ($S_d$) and the previous choice. For each choice $S_i$ with $i \in\{1,2,3\}$, $S_i + S_4 + S_d \rightarrow S_i$ and $S_i + S_4 + S_d \rightarrow S_4$.

    \item We create rules that walk the Hamiltonian path with valid connecting species and a `fuel' species ($P_i$) so that we can only visit a vertex one time. We create each of the rules $S_{i,j,k}$ + $S_{j,k,l} + P_k \rightarrow S_{j,k,l}$ where $i,j,k,l \in V$ and $i\neq t, l \neq s$. This rule essentially says we are walking from $j$ to $k$ along a valid edge and removing the $P_k$ token to note that the vertex has been visited.
\end{itemize}

\paragraph{Example.} For Figure \ref{fig:hamgraph}, we give the full reduction as follows. The final configuration that is only reachable if there is a Hamiltonian path is just the single copy of $S_t$.
\begin{itemize}
    \item The main species are $S_s$, $S_{s,a,b}$, $S_{s,a,c}$, $S_{a,b,c}$, $S_{a,b,t}$, $S_{a,c,d}$, $S_{b,c,d}$, $S_{c,d,t}$, $S_{t}$, $P_a$, $P_b$, $P_c$, $P_d$, and $P_t$. We also create the dummy species $D_{a}$, $D_b$, $D_c$. We have a single copy of each of these.
    \item The tournament reactions for each vertex are (d has only one path)
    \begin{itemize}
        \item a) $S_{s,a,b} + S_{s,a,c} + D_{a}\rightarrow S_{s,a,b}$ and $S_{s,a,b} + S_{s,a,c} + D_{a}\rightarrow S_{s,a,c}$,
        \item b) $S_{a,b,c} + S_{a,b,t} + D_{b}\rightarrow S_{a,b,c}$ and $S_{a,b,c} + S_{a,b,t} + D_{b}\rightarrow S_{a,b,t}$,
        \item c) $S_{a,c,d} + S_{b,c,d} + D_{c}\rightarrow S_{a,c,d}$ and $S_{a,c,d} + S_{b,c,d} + D_{c}\rightarrow S_{b,c,d}$.
        %\item d) Has only one path.
    \end{itemize}
    \item The walking reactions for each vertex are
    \begin{itemize}
        \item a) $S_s + S_{s,a,b} + P_a \rightarrow S_{s,a,b}$ and $S_s + S_{s,a,c} + P_a \rightarrow S_{s,a,c}$,
        \item b) $S_{s,a,b} + S_{a,b,c} + P_b \rightarrow S_{a,b,c}$ and $S_{s,a,b} + S_{a,b,t} + P_b \rightarrow S_{a,b,t}$,
        \item c) $S_{s,a,c} + S_{a,c,d} + P_c \rightarrow S_{a,c,d}$ and $S_{a,b,c} + S_{b,c,d} + P_c \rightarrow S_{b,c,d}$,
        \item d) $S_{a,c,d} + S_{c,d,t} + P_d \rightarrow S_{c,d,t}$ and $S_{b,c,d} + S_{c,d,t} + P_d \rightarrow S_{c,d,t}$,
        \item t) $S_{a,b,t} + S_t + P_t \rightarrow S_t$ and $S_{c,d,t} + S_t + P_t \rightarrow S_t$.
    \end{itemize}
\end{itemize}

\begin{theorem}\label{thm:31npc}
     Reachability for CRNs with only void rules of size $(3, 1)$ is NP-complete, even for unary encoded species counts.
\end{theorem}
\begin{proof}
We reduce from directed Hamiltonian path. Given an instance $H=\langle G,s,t\rangle$ where $G=\{V,E\}$ is a directed graph and $s,t\in V$, is there a Hamiltonian path from $s$ to $t$ in the graph. We convert this to an instance of the reachability problem, as outlined above, to CRN $C$ and the desired configuration $\{S_t:1\}$. We show that $H$ is true iff $\{S_t:1\}$ is reachable in $C$.

\emph{Forward Direction.} Assume there exists a Hamiltonian path in $G$ from $s$ to $t$. Give CRN sequence to get there.

\emph{Reverse Direction.} Assume there exists a reaction sequence in $C$ that reaches the configuration $\{S_t:1\}$. Assume there is a sequence that's not a ham path.
\end{proof}


%%%%%%%%%%%%%
%3,2
%%%%%%%%%%%%%

\begin{theorem}\label{thm:(3,2) rules}
    Reachability for general CRNs with only void rules of size $(3,2)$ is in P.
\end{theorem}
\begin{proof}
    Follows from Theorem \ref{thm:(n,n-1) rules}
\end{proof}

\begin{corollary}\label{cor:32npc}
    Reachability for 2-step CRNs with only void rules of size (3, 2) is NP-complete, even for unary encoded species counts.
\end{corollary}
\begin{proof}
    Follows from Theorem \ref{thm:21npc}.
\end{proof}
\subsection{Size $k$ Void Rules}

We show that reachability is solvable in polynomial time with size $(k, k-1)$ rules. 

%%%%%%%%%%%%%
%n,n-1
%%%%%%%%%%%%%
\begin{lemma}\label{lem:(n,n-1) max rules needed}
    Reachability for general CRNs with only void rules of size $(k, k-1)$ requires at most $|S|$ reactions, where $S$ is the set of species.
\end{lemma}
\begin{proof}
    Let $n = |S|$. Assume there exists a sequence of reactions $a_1r_1,\ldots , a_{n+1}r_{n+1}$ that solves the problem of reachability for some system with set of species $S$ and set of rules $R$, where $a_1, \ldots , a_{n+1}$ are positive integers (denoting how many times to apply each rule) and $r_1, \ldots, r_{n+1}$ are rules in $R$. There must then exist some species $s$ that gets consumed by 2 rules $r_i$ and $r_j$, where $i < j$. Let $s^i$, $s^x$ and $s^f$ denote the initial, intermediate and final counts of species $s$, where $r_i$ reduces $s$ from $s^i$ to $s^x$ and $r_j$ reduces $s$ from $s^x$ to $s^f$. Since $s^i > s^x$, any rule $r_k$, where $k > i$, that uses $s$ with count $s^x$ can also use $s$ with count $s^i$. Thus, rule $r_i$ is not needed. 
\end{proof}
\begin{theorem}\label{thm:(n,n-1) rules}
    Reachability for general CRNs with only void rules of size $(k, k-1)$ is in $P$.
\end{theorem}
\begin{proof}
    For each species $s_j \in S$, create vertex $V^*_j$ to represent this species and let $s_j^i$ represent the initial count and $s_j^f$ represent the final count. Apply rules to reduce each $s_j^i$ to $max(s_j^f, k-1)$ if $s_j^i > k-1$. Otherwise, remove any rule requiring $> s_j^i$ of $s_j$. For each rule in the rule set, introduce a new vertex (if one does not already exist) to represent the catalysts used in the rule (i.e for $A + 2B + C \rightarrow 2B + C$, create vertex $V_{2BC}$). Construct a dependency graph such that for each rule $r \in R$, there exists a directed edge to the vertex representing the species consumed in $r$ from the vertex representing the catalyst(s) it uses. Let $C \subseteq S$ represent a set of species already in their final counts. Repeat the following: 
    \begin{enumerate}
        \item For every vertex $V_L$ in the dependency graph, run a BFS from this vertex if for each $l \in L, l$ is either in $C$ or the final count of $l$ is enough for the reaction to occur.   
        \item For any $V^*_j$ that is marked, append to $C$.
        \item Repeat steps 1 and 2.
    \end{enumerate}
    If $C = S$, then reachability is possible. Otherwise, it is not.  

    By Lemma \ref{lem:(n,n-1) max rules needed}, there exists a sequence of at most $|S|$ reactions which reduces each species from their initial counts to their final counts (without stopping at some intermediate count). Thus, there must exist an ordering of these reactions such that species which get reduced to their final counts with some initial reaction can still allow later reactions to occur. A bottom up approach can be used to find this ordering, starting from the reactions that can occur last to the reactions that must occur first. 

    The dependency graph contains $O(|S| + |R|)$ vertices. Hence, reachability is solvable in polynomial time. 
\end{proof}

\begin{corollary}
    Reachability for general CRNs with only void rules of size $(k_1, k_1-1), \ldots, (k_b, k_b-1)$ is in P.
\end{corollary}
\begin{proof}
    Proof follows from Theorem \ref{thm:(n,n-1) rules}.
\end{proof}

\begin{theorem}
Reachability in interactive step CRNs is PSPACE-hard, with only void rules.
\end{theorem}
\begin{proof}
\textit{UNKNOWN. Alberto and Rachel have been working on it.}
\end{proof}


\begin{corollary}\label{cor:nn-1npc}
    Reachability for 2-step CRNs with only void rules of size $(n, n-1)$, where $n$ is the number of species, is NP-complete, even for unary encoded species counts.
\end{corollary}
\begin{proof}
    Follows from Theorem \ref{thm:21npc}.
\end{proof}
